C-Uniform Trajectory Sampling For Fast Motion Planning

We study the problem of sampling robot trajectories and introduce the notion of C-Uniformity. As opposed to the standard method of uniformly sampling control inputs (which lead to biased samples of the configuration space), C-Uniform trajectories are generated by control actions which lead to uniform sampling of the configuration space. After presenting an intuitive closed-form solution to generate C-Uniform trajectories for the 1D random-walker, we present a network-flow based optimization method to precompute C-Uniform trajectories for general robot systems. We apply the notion of C-Uniformity to the design of Model Predictive Path Integral controllers. Through simulation experiments, we show that using C-Uniform trajectories significantly improves the performance of MPPI-style controllers, achieving up to 40% coverage performance gain compared to the best baseline. We demonstrate the practical applicability of our method with an implementation on a 1/10th scale racer.

==> sections/3-problem_formulation.tex <==
The general problem we would like to solve is the following:

Consider a discrete-time system and let $L = L_i$ and $L' = L_{i+1}$ be any two consecutive level-sets.
Our goal is to assign $p(x, u)$ for each $x \in L$ and $u \in \mathcal{U}$ 

This section provides the problem formulation based on the stochastic optimal control problem.  Therefore, the formulation follows the general optimization scheme, and the objective is to minimize the cost function over sampled trajectories generated by our proposed novel \ourmethod trajectory sampling strategy.
Consider a general vehicle model operating in a state space $\mathcal{X} \subseteq \mathbb{R}^n$, where each state is represented by the vector $\mathbf{x} \in \mathcal{X}$, and $\mathbf{u} \in \mathcal{U} \subseteq \mathbb{R}^m$ is the control input. Thus, the vehicle model can also be defined as Eq. \ref{dynamics}. It is also assumed that the vehicle model can be locally linearizable around a particular operating point. 
Given an initial state $\mathbf{x}_0 \in \mathcal{X}$ and any sequence of control inputs $\mathbf{u}_0, \mathbf{u}_1, \dots, \mathbf{u}_{N-1} \in \mathcal{U}$, the system evolves over $N$ steps according to the dynamics. The SOC problem is formulated as follows:

\begin{equation}
    \begin{aligned}
    \min_{\mathbf{u}_{0:N-1}} & \quad \mathbb{E} \left[ \sum_{t=0}^{N-1} \ell(\mathbf{x}_t, \mathbf{u}_t) + \ell_f(\mathbf{x}_N) \right] \\
    \text{s.t.} & \quad \mathbf{x}_{t+1} = f(\mathbf{x}_t, \mathbf{u}_t) + \mathbf{w}_t, \\
    & \quad \mathbf{x}_t \in \mathcal{X}, \quad \mathbf{u}_t \in \mathcal{U}, \quad \forall t = 0, \dots, N-1
    \end{aligned}
\end{equation}


\subsection{Uniform Reachability Distribution Across Level Sets}
The aim of the proposed method is partitioning the level set $L_{t}$ into $M$ clusters $C_i$ so that the reachability probabilities across these clusters are uniform. To achieve this, it is needed to assign probabilities to the actions $\mathbf{u}_{t-1}$ for a given state $\mathbf{x}_{t-1}$ in the previous level set $L_{t-1}$ so that the distribution of the clusters in $L_{t}$ is uniform. The described problem is formulated as follows:


\begin{align}\label{eq:uniform_prob_state}
&\text{Find} \quad P_{t-1}(\mathbf{u} \mid \mathbf{x}) \\
\text{s.t.} \\
\quad \sum_{\mathbf{u}_{t-1} \in \mathcal{U}} & P_{t-1}(\mathbf{u} \mid \mathbf{x}) = 1, \quad \forall \mathbf{x}_{t-1} \in L_{t-1},\\
&P\left( C_i \right) = \frac{1}{M}, \quad \forall i = 1, \dots, M,\\
&P\left( C_i \right) = \sum_{\mathbf{x}_{t-1} \in L_{t-1}} \sum_{\mathbf{u}_{t-1}:\mathbf{x}_{t},f} P(\mathbf{x}_t) \cdot P_{t-1}(\mathbf{u} \mid \mathbf{x})
\end{align}    


where $P_{t-1}(\mathbf{u} \mid \mathbf{x}) = P(\mathbf{u}_{t-1} \mid \mathbf{x}_{t-1})$ is the probability of choosing an action $\mathbf{u}_{t-1}$ given the state $\mathbf{x}_{t-1}$ in the previous level set, $P(C_i)$ is the probability of the cluster $C_i$ in the current level set, which contains some $\mathbf{x}_{t}$ and $M$ is the total number of clusters. The notation $\mathbf{u}_{t-1}:\mathbf{x}_{t},f $ express the set of actions $\mathbf{u}_{t-1}$, which lead to the $x_t$ with $f(\mathbf{x}_{t-1},\mathbf{x}_{t-1})$. Thus, The goal is to find the action distributions for the $x_{t-1}$ such that the probability of propagating to the new level set $L_t$ with uniform distribution.

